Practical Subtyping for System F with Sized (Co-)Induction

We present a rich type system with subtyping for an extension of System F. Our type constructors include sum and product types, universal and existential quantifiers, inductive and coinductive types. The latter two size annotations allowing the preservation of size invariants. For example it is possible to derive the termination of the quicksort by showing that partitioning a list does not increase its size. The system deals with complex programs involving mixed induction and coinduction, or even mixed (co-)induction and polymorphism (as for Scott-encoded datatypes). One of the key ideas is to completely separate the induction on sizes from the notion of recursive programs. We use the size change principle to check that the proof is well-founded, not that the program terminates. Termination is obtained by a strong normalization proof. Another key idea is the use symbolic witnesses to handle quantifiers of all sorts. To demonstrate the practicality of our system, we provide an implementation that accepts all the examples discussed in the paper and much more.

==> GNUmakefile <==
MAIN  = toplas2017_subtyping
PROTO = /usr/local/bin/subml

GENERATED =\
	munu.tex mitchell.tex scottrec.tex cat.tex  \
	idnat.tex map.tex applist.tex filter.tex

TEXFILES  =\
	$(MAIN).tex abstract.tex algorithm.tex completeness.tex\
	conclusion.tex epsilon.tex interpretation.tex introduction.tex sct.tex\
	semantics.tex subtyping.tex typesystem.tex typingrules.tex compare.tex\
	sntypingrules.tex fixpoint.tex subtyping2.tex applications.tex \
	ordinals.tex macros.tex matrices.tex genabsseq.tex example.tex \
	$(GENERATED)

all: $(MAIN).pdf

$(MAIN).pdf: $(TEXFILES) biblio.bib
	rubber --unsafe -W all --pdf $<

clean:
	rm -f *~ *.log *.aux *.bbl *.blg *.log *.out

distclean: clean
	rm -f $(GENERATED) *dot2tex* $(MAIN).pdf

%.tex: %.typ $(PROTO)
	$(PROTO) --tex-file $@ --quit $<


==> _region_.tex <==
\message{ !name(semantics.tex)}
\message{ !name(semantics.tex) !offset(-2) }
In this section, we build a realizability model that is shown adequate
with our type system. In particular, formulas are interpreted using
sets of strongly normalizing \emph{pure terms}.
\begin{defi} A term is said \emph{pure} when it does not contain choice
operators $\eps_{x\in A}(t \notin B)$. We denote $\pure \subseteq \Lambda$
the set of pure terms.
\end{defi}
\begin{defi}
We say that a pure term $t \in \pure$ is strongly normalizing if there is no
infinite sequence of reduction starting from $t$. We denote $\calN \subseteq
\pure$ the set of strongly normalizing pure terms.
\end{defi}
\begin{defi}
The set $\mathcal{H}$ of head contexts (i.e. terms with a hole in head
position) is generated by the following grammar.
\begin{align*}
  H
  \bnfeq [\,]
  \bnfor H\;t
  \bnfor H.l
  \bnfor \case{H}{(C_i \to t_i)_{i \in I}}
\end{align*}
Given a term $t$ and a head context $H$ we denote $H[t]$ the term formed
by plugging $t$ into the hole of $H$.
\end{defi}
\begin{defi}
We say that a set of pure terms $\Phi \subseteq \pure$ is saturated if the
following conditions hold.
\begin{itemize}
\item If $H[t[x := u]] \in \Phi$ and $u\in\calN$ then $H[(\lambda x.t)\;u] \in\Phi$.
\item If $H[t\;u] \in \Phi$ and for all $i \in I$ we have $t_i \in \calN$, then
      \[H[\case{D\;u}{D \to t \mid (C_i \to t_i)_{i \in I}}] \in \Phi. \]
\item If $H[t] \in \Phi$ and for all $i \in I$ we have $t_i \in \calN$, then
      \[H[\{ l = t; (l_i = t_i)_{i \in I} \}.l] \in \Phi.\]
\end{itemize}
\end{defi}
\begin{lem}\label{nsat}
The set $\calN$ is saturated.
\end{lem}
\begin{proof}
Once standardisation has been proved for the left-to-right ordering on
redexes, the result is immediate. Indeed, if $H[(\lambda x.t)\;u]$ is
not songly normalizable, then there is an infinite reduction in $t$
(then can not be an infinite reduction in $u$) or a standard reduction
that starts by reducing $H[(\lambda x.t)\;u]$ to $H[t[x := u]]$. In
both cases, we get an infinite reduction of $H[t[x := u]]$. The same
reasoning applies to the last two items of the above definition.

Standardisation can be established
from a
theorem by Muller and Wells \cite{wellsmuller}, because our calculus can be encoded as an
orthogonal and fully extended combinatory reduction system. This is
easy because the only reduction rule using bound variables in $\beta$
which is fully extended and all the rule use disjoint set of sympols.

We just
have to check that the left-to-right ordering is a \emph{good redex
ordering}, which is immediate because
\begin{itemize}
\item A redex to the left of a reduced redex is not duplicated nor
  erased.
\item residual of a redex to the left of a reduced redex remains to
  the left of the residual of the other redexes.
\end{itemize}
% The proof of a similar result can be found in
% the work of Karim Nour and Khelifa Saber \cite{nour}, however it is more
% complex due to specific reduction rules for classical logic and commutative
% cuts. Finally, a general framework for proofs using reducibility candidates
% can be found in the work of Colin Riba \cite{riba, ribalong}.
\end{proof}

\begin{defi}\label{nzdef}
The set of neutral terms $\calNZ \subset \pure$ is defined as the smallest
set such that:
\begin{enumerate}
\item for every $\lambda$-variable $x$ we have $x \in \calNZ$,
\item for every $u \in \calN$ and $t \in \calNZ$ we have $t\,u \in \calNZ$,
\item for every $l\in\mathcal{L}$ and $t\in\calNZ$ we have $t.l \in \calNZ$,
\item for every $(C_i, t_i)_{i \in I} \in (\mathcal{C} \times \calN)^I$ and
      $t \in \calNZ$ we have $\case{t}{(C_i \to t_i)_{i \in I}} \in \calNZ$.
\end{enumerate}
\end{defi}
\begin{lem}\label{nzinn}
We have $\calNZ \subseteq \calN$.
\end{lem}
\begin{proof}
Simple induction on the definition of $\calNZ$, using the fact that
the terms of $\calNZ$ never contain a redex in their left branch.
\end{proof}
\begin{defi}
Given two sets $\Phi_1 \subseteq \Lambda$ and $\Phi_2 \subseteq \Lambda$, we
define $(\Phi_1 \to \Phi_2) \subseteq \Lambda$ as follows.
$$\Phi_1\to\Phi_2 = \{t\in\Lambda \st \forall u\in\Phi_1,\;t\;u \in \Phi_2\}$$
\end{defi}
\begin{lem}\label{inclusion}
Let $\Phi_1$, $\Phi_2$, $\Psi_1$, $\Psi_2 \subseteq \Lambda$ be sets of terms
such that $\Phi_2 \subseteq \Phi_1$ and $\Psi_1 \subseteq \Psi_2$.
We have $(\Phi_1 \to \Psi_1) \subseteq (\Phi_2 \to \Psi_2)$.
\end{lem}
\begin{proof}
Immediate by definition.
% We take $t \in (\Phi_1 \to \Psi_1)$ and show $t \in (\Phi_2 \to \Psi_2)$. By
% definition we know that if $u \in \Phi_1$ then $t\;u \in \Psi_1$. Let us now
% take $u \in \Phi_2$. By hypothesis $u \in \Phi_1$ and hence $t\;u \in \Psi_1$.
% We finally obtain $t\;u \in \Psi_2$ by hypothesis.
\end{proof}
\begin{lem}\label{nnzero}
We have $\calNZ \subseteq (\calN \to \calNZ) \subseteq (\calNZ \to \calN)
\subseteq \calN$.
\end{lem}
\begin{proof}
By Lemma \ref{nzinn} we know that $\calNZ \subseteq \calN$ and hence we
obtain $(\calN \to \calNZ) \subseteq (\calNZ \to \calN)$ using Lemma
\ref{inclusion}. If we take $t \in \calNZ$, then by definition $t\,u \in
\calNZ$ for every $u \in \calN$. Therefore we obtain $\calNZ \subseteq
(\calN \to \calNZ)$. Finally, if we take $t \in (\calNZ \to \calN)$ then
by definition $t\;x \in \calN$ since $x \in \calNZ$. Hence $t \in \calN$,
which gives us $(\calNZ \to \calN) \subseteq \calN$.
\end{proof}

We first need to give the
domain of interpretation for each of the three syntactic category.
\begin{itemize}
\item A closed term $t \in \Lambda$ is interpreted by a pure term
      $\sem{t} \in \pure$. We therefore interpret terms with
      choice operators using (possibly open) pure terms.
\item A formula $A \in \mathcal{F}$ is interpreted by a saturated set of
      pure terms $\sem{A}$ such that $\calNZ \subseteq \sem{A} \subseteq
      \calN$. We denote $\formsem$ the set of every such type
      interpretation.
      $$ \formsem = \{\Phi \subseteq \pure \st \Phi\;\text{saturated},\;
         \calNZ \subseteq \Phi \subseteq \calN\} $$
\item A syntactic ordinal $\kappa \in \mathcal{O}$ will be interpreted by
      an ordinal $\sem{\kappa} \in \ordsem$.
\end{itemize}

To simplify the definition of the semantics, the syntax of terms,
formulas and ordinals is extended with elements of their respective
models. This avoids to always carry the interpretation function giving
the value of the free variables.
\begin{defi}\label{paramdef}
The sets of \emph{parametric} terms, formulas and ordinals are formed by
extending the syntax of ordinals with the elements of $\ordsem$ and the
syntax of formulas with the elements of $\formsem$. The corresponding sets
will be denoted $\parterm$, $\parform$ and $\parord$. Terms do not need to
be extended directly. However, the definition of $\parform$ and $\parord$
impacts the definition of $\parterm$ since terms and formulas are defined
mutually inductively.
\end{defi}

\begin{defi}
A closed parametric term (resp. formula, resp. syntactic ordinal) is a
parametric term (resp. formula, resp. ordinal) with no free type
variables and no free ordinal variables.
\end{defi}

\begin{defi}
The semantics $\sem{t}$ (resp. $\sem{\kappa}$, resp. $\sem{A}$) of a
closed parametric term $t\in\parterm$ (resp. ordinal $\kappa\in\parord$,
resp. type $A\in\parform$) is defined in Figure \ref{interpr}. The
semantics of terms and types need to be defined mutually inductively
because of the choice operators.
\input{interpretation.tex}
\end{defi}
Note that the semantical interpretation of syntactic ordinals is
straightforward because they mostly denote variables, which are not
interpreted directly. Indeed, closed parametric object are built from
non-parametric ones by substituting their free variables with closed
parametric objects (e.g. elements of the semantics). As ordinal variables
carry constraints, we will need to restrict ourselves to substitutions
satisfying these constraints (see Definition \ref{def:acceptable}).

In the interpretation of a choice operators $\eps_{x \in A}(t \notin B)$,
it is important that no $\lambda$-variable other that $x$ is bound in $t$.
This is enforced by a syntactic restriction that was given in Definition
\ref{def:terms}. It is absolutely necessary to obtain a well-defined term
model. Without this restriction, a term  $\sem{\lambda y.\eps_{x \in A}(t
\notin B)}$ with $y$ free in $t$ or $B$ would correspond to a function
that is not always definable using a pure term. In this case, our model
would have circular and hence invalid definitions. Note that the axiom of
choice is required to interpret the choice operators for terms and types.

\begin{lem}\label{th:substitution}
Let $t, u$ be two terms, $\tau, \kappa$ be two syntactic ordinals and
$A, B$ be two types. Let us assume that these are closed parametric with the exception of
$x,\alpha,X$ that may be free in $t$, $\kappa$ and $A$ only (TODO: MAL
DIT, C'EST un à la fois). Then, we
have
\begin{itemize}
\item $\sem{t[x:=u]} = \sem{t[x:=\sem{u}]}$
\item $\sem{t[\alpha:=\tau]} = \sem{t[\alpha:=\sem{\tau}]}$
\item $\sem{t[X:=B]} = \sem{t[X:=\sem{B}]}$
\item $\sem{\kappa[x:=u]} = \sem{\kappa[x:=\sem{u}]}$
\item $\sem{\kappa[\alpha:=\tau]} = \sem{\kappa[\alpha:=\sem{\tau}]}$
\item $\sem{\kappa[X:=B]} = \sem{\kappa[X:=\sem{B}]}$
\item $\sem{A[x:=u]} = \sem{A[x:=\sem{u}]}$
\item $\sem{A[\alpha:=\tau]} = \sem{A[\alpha:=\sem{\tau}]}$
\item $\sem{A[X:=B]} = \sem{A[X:=\sem{B}]}$
\end{itemize}
\end{lem}

\begin{proof}
Immediate by induction on the definition of the semantics.
\end{proof}

\begin{thm}\label{th:semantics}
For every closed parametric term $t \in \parterm$ (resp. ordinal $\kappa
\in \parord$, resp. type $A \in \parform$) we have $\sem{t} \in \pure$
(resp. $\sem{\kappa} \in \ordsem$, resp. $\sem{A} \in \formsem$).
\end{thm}
\begin{proof}
We do a proof by induction. For terms, all the cases are immediate by
induction hypothesis. If $u = \sem{\eps_{x \in A}(t \notin B)}$ then
we have $u \in \calN \subseteq \pure$ since $\calNZ \subseteq \calN$ by
Lemma \ref{nzinn} and $\sem{A} \subseteq \calN$ by induction hypothesis.
For ordinals, the proof is immediate by definition and induction hypothesis.
The saturation is easy for types because the closure of the
definition by head context is exactly what is needed.
For the inclusions, using lemma \ref{nsat}
we obtain $\calN \in \formsem$, hence the proof is immediate for types of
the forms $\Phi$, $\{\}$, $\eps_X(t \in A)$ or $\eps_X(t \notin A)$.
The remaining cases are given below.
% FIXME saturation pour les cas suivants
\begin{itemize}
\item If it is of the form $A \Rightarrow B$, then we have
      $\calNZ \subseteq \sem{A} \subseteq \calN$ and
      $\calNZ \subseteq \sem{B} \subseteq \calN$ by induction hypothesis.
      We need to show that $\calNZ \subseteq \sem{A \to B} \subseteq \calN$.
      By Lemma \ref{nnzero}, it is enough to show
      $(\calN\to\calNZ) \subseteq \sem{A \to B} \subseteq (\calNZ\to\calN)$.
      We can hence conclude using Lemma \ref{inclusion}.
\item If it is of the form $\{(l_i : A_i)_{i \in I \neq \emptyset}\}$ then we
      know that for all $i \in I$ we have $\calNZ \subseteq \sem{A_i}
      \subseteq \calN$ by induction hypothesis. Let us take $t \in \calNZ$
      and show that $t \in \sem{\{(l_i : A_i)_{i \in I \neq \emptyset}\}}$. We
      take $j \in I \neq \emptyset$ and show that $t.l_j \in \sem{A_j}$. It is
      enough to show that $t.l_j \in \calNZ$, which follows by definition of
      $\calNZ$. Let us now take $t \in \sem{\{(l_i : A_i)_{i \in I \neq
      \emptyset}\}}$ and show that $t \in \calN$. Since $I \neq \emptyset$ we
      can take $j \in I$ and by definition $t.l_j \in \sem{A_j} \subseteq
      \calN$. Since $t.l_j$ is strongly normalizing $t$ must be strongly
      normalizing.
\item If it is of the form $[(C_i : A_i)_{i \in I}]$ then we know that for
      all $i \in I$ we have $\calNZ \subseteq \sem{A_i} \subseteq \calN$ by
      induction hypothesis. Let us take $t \in \calNZ$ and show that $t \in
      \sem{[(C_i : A_i)_{i \in I}]}$. Let us now take $\Phi \in \formsem$ and
      $(t_i \in (\sem{A_i} \to \Phi))_{i \in I}$ and show that
      $\case{t}{(C_i \to t_i)_{i \in I}} \in \Phi$. It is enough to show that
      $\case{t}{(C_i \to t_i)_{i \in I}} \in \calNZ$ and since $t \in \calNZ$
      we only have to show $t_i \in \calN$ for all $i \in I$, by definition
      of $\calNZ$. It is the case since
      $(\sem{A_i} \to \Phi) \subseteq (\calNZ \to \calN) \subseteq \calN$ by
      Lemmas \ref{inclusion} and \ref{nnzero}. Let us now take
      $t \in \sem{[(C_i : A_i)_{i \in I}]}$ and show that $t \in \calN$. Let
      us take take $\Phi \in \formsem$ and $(t_i \in \sem{A_i} \to
      \Phi)_{i \in I}$. By definition $\case{t}{(C_i \to t_i)_{i \in I}} \in
      \Phi \subseteq \calN$, hence we must have $t \in \calN$.
\item If it is of the form $\forall X. A$ or $\exists X. A$ then for every
      $\Phi \in \formsem$ we have $\calNZ \subseteq \sem{A[X := \Phi]}
      = \subseteq \calN$ by induction hypothesis. As a consequence we obtain
      that $\calNZ \subseteq \sem{\forall X. A} \subseteq \calN$ and
      that $\calNZ \subseteq \sem{\exists X. A} \subseteq \calN$.
\item If it is of the form $\mu_\kappa X. A$ or $\nu_\kappa X. A$, we
  prove that $\calNZ \subseteq \sem{\mu_o X. A} \subseteq \calN$ for
  $o \leq \sem{\kappa}$ by induction on the ordinal $o$. If
  $o = 0$, this is immediate as $\sem{\mu_0 X. A} = \calNZ$.
   Otherwise, $\sem{\mu_o X. A} =
   \cup_{o' < o} \sem{A[X:=\mu_{o'} X. A]}$. We have
   $\sem{A[X:=\mu_{o'} X. A]} = \sem{A[X:=\sem{\mu_{o'} X. A}]}$.
by lemma \ref{th:substitution}.
  By induction hypothesis on $o'$, we have $\calNZ \subseteq
  \sem{\mu_{o'} X. A} \subseteq \calN$ hence  $\calNZ \subseteq
  \sem{A[X:=\sem{\mu_{o'} X. A}]} \subseteq \calN$ by induction
  hypothesis on $A$. The case of $\nu_\kappa X. A$ is identical.
\end{itemize}
\vspace{-4.1ex}
\end{proof}

\begin{defi}\label{def:acceptable}
A substitution $\sigma$ for terms, ordinals and type variables is said to be
acceptable for some terms, ordinals and types if after substitution, the resulting terms,
ordinals and types are closed parametric.
\end{defi}

\begin{thm}\label{th:adequacy}
Let $A$ and $B$ be types, $t$ be a term and $\sigma$ be an acceptable
substitution for $t$, $A$ and $B$.
\begin{itemize}
\item If $\type{t}{A}$ is derivable then $\sem{t\sigma} \in \sem{A\sigma}$.
\item Let assume that for all $\kappa \in \gamma$ a finite set of
  syntactic ordinals, we have $\kappa\sigma >0$. If $\subtype{\gamma}{t}{A}{B}$  is derivable and $\sem{t\sigma} \in \sem{A\sigma}$ then $\sem{t\sigma} \in \sem{B\sigma}$.
\end{itemize}
\end{thm}
\begin{proof}
We do a proof by induction on the derivations. Let us first note that if
$\kappa < \tau$ (resp. $\kappa \leq \tau$) is derivable then
$\sem{\kappa\sigma} < \sem{\kappa\sigma}$ (resp. $\sem{\kappa\sigma} \leq
\sem{\kappa\sigma}$) follows from the definition of acceptable substitution,
provided that $\sigma$ is acceptable for $\kappa$ and $\tau$.
%
For subtyping proof that can be cyclic

We now reason by case analysis on the last typing or local subtyping rule used
in the derivation of the considered typing or local subtyping judgment.
\begin{itemize}
\item[$\epsilon$] Let $\sigma$ be an acceptable substitution for $t$, $A$,
  $B$ and $C$. By definition of $u = \sem{\epsilon_{x\in A\sigma}(t\sigma
  \notin B\sigma)} \in \sem{A\sigma}$, and hence $u \in \sem{C\sigma}$ by
  induction hypothesis
\item[$\to_i$] Let $\sigma$ be an acceptable substitution for $\lambda x.t
  \in C$. We need to show that $\sem{(\lambda x t)\sigma} \in \sem{C\sigma}$.
  We can assume that $\sigma$ is acceptable with $A \to B$, because
  $\sem{(\lambda x t)\sigma}$ and $\sem{C\sigma}$ are independent of
  $\alpha\sigma$ for any ordinal $\alpha$ that occurs in $A \to B$ but not
  in $C$, nor in $t$. Therefore, by induction hypothesis, we have
  $\sem{(\lambda x t)\sigma} \in \sem{(A \to B)\sigma}$ implies
  $\sem{(\lambda x t)\sigma} \in \sem{C\sigma}$. It remains to prove
  that $\sem{(\lambda x t)\sigma} \in \sem{(A \to B)\sigma}$. By
  induction hypothesis, we have
  $\sem{t\sigma[x:=\epsilon_{x\in A\sigma}(t\sigma \notin B\sigma)]} \in
  \sem{B\sigma}$
  which by definition of the choice operator means that for all
  $u \in \sem{A\sigma}$ we have $\sem{t\sigma[x:=u]} \in \sem{B\sigma}$.
\item[$\forall_r$] Let $\sigma$ be an acceptable substitution for
  $\subtype{t}{A}{\forall X. B}$. We assume $\sem{t\sigma} \in \sem{A\sigma}$
  and show $\sem{t\sigma} \in \sem{(\forall X. B)\sigma}$. Up to a renaming
  of $X$, we may assume that $(\forall X. B)\sigma = \forall X. B\sigma$.
  By induction hypothesis $\sem{t\sigma} \in \sem{B\sigma[X := \epsilon_X(t
  \sigma \notin B\sigma)]}$ and hence $\sem{t\sigma} \in \sem{A\sigma}$.
  Consequently we $\sem{t\sigma} \in \sem{B\sigma[X := \Phi]}$ for all $\Phi
  \in \formsem$ by definition of the choice operator. We hence obtain
  $\sem{t\sigma} \in \sem{(\forall X. B)\sigma}$.
\item[$\mu_l^*$] Let sigma be an acceptable substitution for
  $\subtype{t}{\mu_\kappa X. A}{B}$. We assume $\sem{t\sigma} \in
  \sem{(\mu_\kappa X. A)\sigma}$ and $(\mu_\kappa X. A)\sigma =
  \mu_\kappa X. A\sigma$ (renaming $X$ if necessary). By definition,
  this means that we can find $o < \sem{\kappa\sigma}$ such that
  $\sem{t\sigma} \in \sem{A\sigma[X := \mu_o X. A\sigma]}$. The
  substitution $\rho = \sigma[\alpha := o]$ is acceptable for
  $t$, $B$ and $A[X := \mu_{\alpha_{<\kappa}} X. A$. Furthermore
  we have $t \rho = t\sigma$, $A\rho=A\sigma$ and $B\rho=B\sigma$ because
  of the constraint on $\alpha$. As a consequence,
  $\sem{t\sigma} \in \sem{B\rho} = \sem{B\sigma}$ by induction hypothesis.
\item[$I_m$] The intuition for the induction rules is given informally in
  the previous section. One point is missing to make the argument formal:
  the fact that the semantical truth of $\subt{A\sigma}{B\sigma}$ for
  an acceptable substitution $\sigma$ indeed implies $\sem{A\sigma} \subset
  \sem{B\sigma}$. By definition, the truth of the judgment means that
  $u = \sem{\epsilon_{x \in A\sigma}(x \notin B\sigma)} \in \sem{A\sigma}$
  implies $u \in \sem{B\sigma}$. By definition of the semantics of the
  choice operator, this implication can only be true if $\sem{A\sigma}
  \subset \sem{B\sigma}$, otherwise we would obtain a contradiction with
  $u \in \sem{A\sigma}$ and $u \notin \sem{A\sigma}$.
\end{itemize}
The remaining cases can be proved in a similar way.
\end{proof}

% Strong normalization
The previous theorem is generally called the \emph{adequacy lemma}.
Intuitively, it establishes the compatibility between the syntax and
the semantics. We will now rely on this theorem to obtain results
such as strong normalization.
\begin{thm}\label{th:strongnorm}
Let $t$ be a pure term. If there is a type $A$ with no free ordinal
variables such that $\type{t}{A}$ then $t$ is strongly normalizable.
\end{thm}
\begin{proof}
We consider the substitution $\sigma$ mapping all the free type
variables of $A$ to $\calN$. It is obviously acceptable for $t$
and $A$. Indeed, $t$ cannot contain types or semantic ordinals as
it is pure. Using the adequacy lemma (Theorem \ref{th:adequacy}),
we obtain that $\sem{t\sigma} \in \sem{A\sigma}$. We hence get
$t \in \sem{A\sigma} \subseteq \calN$ using Theorem \ref{th:semantics}.
\end{proof}
%
A direct consequence of strong normalization is that well-typed terms
cannot produce runtime errors thanks to our definition of reduction.

\begin{thm}\label{th:safety}
We say that a data type is simple if it is closed and only contains sums,
products and fixpoints. If we can derive $t:A$ for a simple data type $A$
and a closed pure term $t$, then $t$ reduces to a normal form $u$ and
$\type{u}{A}$ is derivable.
\end{thm}
\begin{proof}
Using strong normalization (Theorem \ref{th:strongnorm}) we know that
$t$ reduces to a normal form $u$ that remains closed (no free variables
are introduced during reduction). Since $A$ is a simple datatype, we can
show by induction on $A$ that $u \in \sem{A}$ implies $\type{u}{A}$
if $u$ is in normal form.
\end{proof}

\begin{thm}[logical consistency]\label{th:consistency}
There is no closed term $t$ such that we can derive
$\type{t}{\forall X.X}$ or $\type{t}{[\,]}$.
\end{thm}
\begin{proof}
This result follows from Theorem \ref{th:adequacy} using the fact that
$\sem{\forall X.X} = \sem{[\;]} = \calNZ$ only contains open terms.
\end{proof}

\message{ !name(semantics.tex) !offset(-404) }


==> attic.tex <==
For instance, OCaml's polymorphic variants \cite{polyvar} require specific
annotations on the corresponding sum types. For example, one would expect the
following boolean negation function to have type
\verb#[`T|`F]# $→$ \verb#[`T|`F]#.
\smallskip
\begin{center}
  \verb#fun x# $→$ \verb#match x with `T# $→$ \verb#`F | `F# $→$ \verb#`T#
\end{center}
\smallskip
Indeed, the variance of the arrow type conveys enough information: the
function can be applied to elements of any subtype of \verb#[`T|`F]#, for
example \verb#[`T]#, to produce elements of any supertype of \verb#[`T|`F]#,
for example \verb#[`T|`F|`M]#.
%
In practice, OCaml infers the type \verb#[<`T|`F]# $→$ \verb#[>`T|`F]# in
which subtypes and supertypes are explicitly tagged. This is not very natural
and hides a complex mechanism involving polymorphic type variables.



==> completeness.tex <==
We give a completeness result for the system without implication, universal and
existential quantification. We also discuss completeness with
implication at the end.

\begin{thm}
  The typing and subtyping algorithms give in the previous section, restricted to
  formulas without universal nor existential quantification
\end{thm}

\begin{thm}
  Let $A$ and $B$ be two formulas without implication, universal nor
  existential quantification. We have
\[ \vdash A \subset B \hbox{ iff } \forall \sigma, \sem{A\sigma} \subset \sem{B\sigma} \]
\end{thm}

\begin{proof}
\dots
\end{proof}

\begin{thm}
Let $t$ be a term and $A$ a type without implication, universal nor
existential quantification. We have
\[ \vdash t : A \hbox{ iff } \forall \sigma, t\sigma \in \sem{A\sigma} \]
\end{thm}

\begin{proof}
\dots
\end{proof}

We believe that completeness in presence of implication is true, but
probably not for one model, but for a family of model. Indeed, when
$A \to B \subset C \to D$ is not provable, it means that either
$C \subset A$ or $B \subset D$ is not provable. In the case
when $B \subset D$ is provable but $C \subset A$ is not, the induction
hypothesis in an hypothetical completeness proof would give a
term $u \in \sem{C}$ such that $u \not\in \sem{A}$. Then, if we consider the
``term'' $t = \lambda y (\hbox{ if } x \equiv u \hbox{ then } z \hbox{
  else } \Omega)$,
where $z$ is a free variable and $\Omega$ any non strongly normalising
term, assuming a reasonnable semantics for the condition, we would
prove that $t \in \sem{A \to B}$, but $t \notin \sem{C \to D}$,
if $t(u) \equiv \Omega$ and the semantics is closed by equivalence.

We think that this argument can be made concrete with the techniques in
\cite{lepigre}.

%%% Local Variables:
%%% ispell-personal-dictionary: "~/.hunspell-en"
%%% ispell-local-dictionary: "british"
%%% End:


==> insert_sort.tex <==

We can also prove termination and preservation of size for the insertion sort.
\begin{align*}
\mathrm{F}(A,X) &= [\mathrm{Nil} | \mathrm{Cons} \of \{\mathrm{hd} : A; \mathrm{tl} : X\}]\\
\mathrm{insert} &\,: ∀α.∀A.(A → A → \mathbb{B}) → A → \mathbb{L}_{α}(A) → \mathbb{L}_{α+1}(A)\\ &= Yinsert.λf\, a\, l.\casearray{l}{\begin{array}{l} [] → a{::}[] \\ x::l → \case{f \; a \; x}{ T → a{::}l ∣ F → x{::}insert \; f \; a \; l}\end{array}}\\
\mathrm{sort} &\,: ∀α.∀A.(A → A → \mathbb{B}) → \mathbb{L}_{α}(A) → \mathbb{L}_{α}(A)\\ &= Ysort.λf\, l.\casearray{l}{\begin{array}{l} [] → [] \\ x::l → \mathrm{insert} \; f \; x \; (sort \; f \; l)\end{array}}\\
\end{align*}

We also tested the quick sort and merge sort and in both case managed to prove termination, but not size preservation. Proving size preservation of such programs would probably be possible
is the language for ordinals were extended with an addition symbol, which would allow to give a precise type to functions splitting a list in two parts while keeping a constant total size.


==> integer.tex <==

\subsection*{Typable recursor.}
We are now going to exhibit some short but enlightening examples
showing the power of our system. The first examples are Church and
Scott encodings of natural numbers. Although they have little
practical interest, they provide difficult tests because they
rely heavily on polymorphism and fixpoints. The type of Church
natural numbers $\mathbb{N}_C$ and the type of Scott natural numbers
$\mathbb{N}_S$ are defined below, together with their respective
zero and successor functions.

\begin{align*}
\mathbb{N}_C &= ∀X.(X → X) → X → X\\
0_C &: \mathbb{N}_C = λf\, x.x \\
S_C &: \mathbb{N}_C → \mathbb{N}_C = λn\, f\, x.f \; (n \; f \; x) \\
\mathbb{N}_S &= μN.∀X.(N → X) → X → X\\
0_S &: \mathbb{N}_S = λf\, x.x \\
S_S &: \mathbb{N}_S → \mathbb{N}_S = λn\, f\, x.f \; n
\end{align*}

Using Church encoding, our algorithm is able to typecheck the usual
terms for predecessor $P_C$, recursor $R_C$, but also the
less usual Maurey infimum $ (\leq) $, which requires inductive type
\cite{krivine}. It can be typechecked giving only the type
to use for the natural number: $N_t = (\mathrm{T} → \mathrm{T}) → \mathrm{T} → \mathrm{T}$ where $\mathrm{T} = μX.((X → \mathbb{B}) → \mathbb{B})$.
They are defined as follows, where $T,F :  \mathbb{B} $ denote booleans.
\begin{align*}
P_C     &: \mathbb{N}_C → \mathbb{N}_C = λn.n \; (λp\, x{:}\mathbb{N}_C\, y{:}\mathbb{N}_C.p \; (S_C \; x) \; x) \; (λx\, y.y) \; 0_C \; 0_C \\
R_C &: ∀P.(P → \mathbb{N}_C → P) → P → \mathbb{N}_C → P\\ &= λf\, a\, n.n \; (λx\, p{:}\mathbb{N}_C.f \; (x \; (S_C \; p)) \; p) \; (λp.a) \; 0_C \\
 (\leq)      &= \mathbb{N}_C → \mathbb{N}_C →  \mathbb{B} \\ &= λn\, m.(n : N_t) \; (λf\, g.g \; f) \; (λi.T) \; ((m : N_t) \; (λf\, g.g \; f) \; (λi.F))
\end{align*}

Scott numerals were introduced because they have a constant time
predecessor, whereas Church numerals don't. Usually, programming
using Scott numerals require the use of recursor in the style of
Gödel's System T. Such a recursor can be programmed using a general
fixpoint combinator, however this would imply the introduction of
typable terms that are not strongly normalizing. In our type system,
we can typecheck a strongly normalisable recursor found by Michel
Parigot\cite{parigotX}. It is displayed below together with several other terms
and types that are used for Scott encoding.

\begin{align*}
\mathrm{pred} &: \mathbb{N}_S → \mathbb{N}_S = λn.n \; (λp.p) \; 0_S  \\
\mathrm{U}(P) &= ∀Y.Y → \mathbb{N}_S → P \\
\mathrm{T}(P) &= ∀Y.(Y → \mathrm{U}(P) → Y → \mathbb{N}_S → P) → Y → \mathbb{N}_S → P \\
 \mathbb{N}'  &= ∀P.\mathrm{T}(P) → \mathrm{U}(P) → \mathrm{T}(P) → \mathbb{N}_S → P \\
 \zeta  &\,: ∀P.P → \mathrm{U}(P) = λa\, r\, q.a\\
 \delta  &\,: ∀P.P → (\mathbb{N}_S → P → P) → \mathrm{T}(P) \\ &= λa\, f\, p\, r\, q.f \; (\mathrm{pred} \; q) \; (p \; r \; ( \zeta  \; a) \; r \; q) \\
 R_S  &\,: ∀P.P → (\mathbb{N}_S → P → P) → \mathbb{N}_S → P \\ &= λa\, f\, n.(n :  \mathbb{N}' ) \; ( \delta  \; a \; f) \; ( \zeta  \; a) \; ( \delta  \; a \; f) \; n \\
\end{align*}
It is easy to check that the term $ R_S $ is indeed a recursor for
Scott numerals. The term is similar to a fixpoint combinator, with a limited number of steps of recursion. As this term is typable, Theorem \ref{th:strongnorm}
implies that it is strongly normalizable.
%
It can be typechecked because the subtyping relation $ \mathbb{N}_S \subset  \mathbb{N}'  $
holds in our system. It is however not clear what are the terms of type
$ \mathbb{N}' $. The minimum type annotation for our
algorithm to type-check the recursor are its type and the annotation
$n :  \mathbb{N}' $. It is not necessary to give the type of the subterms $ \zeta $
nor $ \delta $.

%%% Local Variables:
%%% ispell-personal-dictionary: "~/.hunspell-en"
%%% ispell-local-dictionary: "british"
%%% End:


==> lmcs_subtyping-dot2tex-fig1.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%

%
\end{tikzpicture}


==> lmcs_subtyping-dot2tex-fig2.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (N0) at (40.243bp,111.06bp) [draw,ellipse] {$g$};
  \node (N1) at (40.243bp,18.057bp) [draw,ellipse] {$f$};
  \draw [->] (N0) ..controls (24.031bp,100.88bp) and (10.067bp,91.025bp)  .. (4.2433bp,78.057bp) .. controls (-1.2188bp,65.893bp) and (-1.5123bp,60.084bp)  .. (4.2433bp,48.057bp) .. controls (8.2382bp,39.709bp) and (15.938bp,32.997bp)  .. (N1);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (30.243bp,63.057bp) node {$\left(\begin{smallmatrix}\infty&0&\infty\cr
0&\infty&\infty\end{smallmatrix}\right)$};
  \draw (26.756bp,100.04bp) node {$$};
  \draw (25.838bp,29.001bp) node {$$};
  \draw [->] (N1) ..controls (49.638bp,32.319bp) and (54.235bp,40.261bp)  .. (56.243bp,48.057bp) .. controls (59.569bp,60.969bp) and (59.307bp,65.08bp)  .. (56.243bp,78.057bp) .. controls (54.955bp,83.512bp) and (52.587bp,89.098bp)  .. (N0);
  \draw (83.243bp,63.057bp) node {$\left(\begin{smallmatrix}\infty&-1\cr
0&\infty\cr
-1&\infty\end{smallmatrix}\right)$};
  \draw (51.885bp,32.722bp) node {$$};
  \draw (38.946bp,97.053bp) node {$$};
  \draw [->] (N0) ..controls (55.96bp,122.48bp) and (66.743bp,120.43bp)  .. (66.743bp,111.06bp) .. controls (66.743bp,105.05bp) and (62.318bp,102.05bp)  .. (N0);
  \draw (97.243bp,111.06bp) node {$\left(\begin{smallmatrix}0&\infty&\infty\cr
\infty&0&\infty\cr
\infty&-1&-1\end{smallmatrix}\right)$};
  \draw (53.031bp,123.21bp) node {$$};
  \draw (53.031bp,98.904bp) node {$$};
  \draw [->] (N1) ..controls (56.906bp,28.411bp) and (67.243bp,26.393bp)  .. (67.243bp,18.057bp) .. controls (67.243bp,12.847bp) and (63.205bp,10.104bp)  .. (N1);
  \draw (89.743bp,18.057bp) node {$\left(\begin{smallmatrix}0&\infty\cr
\infty&-1\end{smallmatrix}\right)$};
  \draw (53.982bp,18.113bp) node {$$};
  \draw (53.982bp,6.0bp) node {$$};
%
\end{tikzpicture}


==> lmcs_subtyping-dot2tex-fig3.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (N0) at (113.71bp,350.25bp) [draw,ellipse] {$cmp_{0}$};
  \node (N1) at (35.708bp,233.75bp) [draw,ellipse] {$cmp_{1}$};
  \node (N2) at (35.708bp,19.748bp) [draw,ellipse] {$cmp_{2}$};
  \node (N3) at (121.71bp,126.75bp) [draw,ellipse] {$cmp_{3}$};
  \draw [->] (N3) ..controls (121.25bp,102.49bp) and (118.4bp,73.582bp)  .. (103.71bp,55.248bp) .. controls (93.382bp,42.364bp) and (76.976bp,33.845bp)  .. (N2);
  \definecolor{strokecol}{rgb}{0.0,0.0,0.0};
  \pgfsetstrokecolor{strokecol}
  \draw (150.21bp,73.248bp) node {$\left(\begin{smallmatrix}0&\infty&\infty\cr
\infty&0&\infty\cr
\infty&-1&\infty\cr
\infty&\infty&-1\end{smallmatrix}\right)$};
  \draw (115.7bp,110.93bp) node {$$};
  \draw (59.117bp,19.144bp) node {$$};
  \draw [->] (N2) ..controls (29.152bp,43.753bp) and (23.858bp,72.453bp)  .. (36.708bp,91.248bp) .. controls (37.631bp,92.599bp) and (72.404bp,106.44bp)  .. (N3);
  \draw (70.208bp,73.248bp) node {$\left(\begin{smallmatrix}0&\infty&\infty&\infty\cr
\infty&0&\infty&\infty\cr
\infty&\infty&\infty&0\end{smallmatrix}\right)$};
  \draw (39.009bp,35.463bp) node {$$};
  \draw (100.74bp,113.92bp) node {$$};
  \draw [->] (N3) ..controls (146.98bp,138.78bp) and (160.71bp,136.19bp)  .. (160.71bp,126.75bp) .. controls (160.71bp,119.81bp) and (153.31bp,116.58bp)  .. (N3);
  \draw (189.71bp,126.75bp) node {$\left(\begin{smallmatrix}0&\infty&\infty\cr
\infty&0&\infty\cr
\infty&\infty&-1\end{smallmatrix}\right)$};
  \draw (128.49bp,140.5bp) node {$$};
  \draw (140.49bp,113.0bp) node {$$};
  \draw [->] (N2) ..controls (60.983bp,31.776bp) and (74.708bp,29.193bp)  .. (74.708bp,19.748bp) .. controls (74.708bp,12.812bp) and (67.306bp,9.5764bp)  .. (N2);
  \draw (111.71bp,19.748bp) node {$\left(\begin{smallmatrix}0&\infty&\infty&\infty\cr
\infty&0&\infty&\infty\cr
\infty&-1&-1&\infty\cr
\infty&\infty&\infty&0\end{smallmatrix}\right)$};
  \draw (54.491bp,33.496bp) node {$$};
  \draw (54.491bp,6.0bp) node {$$};
  \draw [->] (N0) ..controls (149.77bp,340.88bp) and (175.67bp,330.97bp)  .. (187.71bp,311.25bp) .. controls (200.26bp,290.69bp) and (217.18bp,212.38bp)  .. (186.71bp,162.25bp) .. controls (178.49bp,148.72bp) and (162.99bp,140.2bp)  .. (N3);
  \draw (242.71bp,233.75bp) node {$\left(\begin{smallmatrix}0&\infty&\infty&\infty&\infty\cr
\infty&\infty&0&\infty&\infty\cr
\infty&\infty&\infty&\infty&0\end{smallmatrix}\right)$};
  \draw (138.04bp,351.54bp) node {$$};
  \draw (145.58bp,137.81bp) node {$$};
  \draw [->] (N3) ..controls (81.363bp,143.23bp) and (32.984bp,161.84bp)  .. (32.708bp,162.25bp) .. controls (22.347bp,177.38bp) and (25.127bp,198.91bp)  .. (N1);
  \draw (64.208bp,180.25bp) node {$\left(\begin{smallmatrix}0&\infty&\infty\cr
-1&\infty&\infty\cr
\infty&0&\infty\cr
\infty&\infty&-1\end{smallmatrix}\right)$};
  \draw (100.67bp,139.52bp) node {$$};
  \draw (38.27bp,218.03bp) node {$$};
  \draw [->] (N1) ..controls (60.983bp,245.78bp) and (74.708bp,243.19bp)  .. (74.708bp,233.75bp) .. controls (74.708bp,226.81bp) and (67.306bp,223.58bp)  .. (N1);
  \draw (111.71bp,233.75bp) node {$\left(\begin{smallmatrix}0&\infty&\infty&\infty\cr
-1&-1&\infty&\infty\cr
\infty&\infty&0&\infty\cr
\infty&\infty&\infty&0\end{smallmatrix}\right)$};
  \draw (42.491bp,247.5bp) node {$$};
  \draw (54.491bp,220.0bp) node {$$};
  \draw [->] (N0) ..controls (67.843bp,346.58bp) and (26.264bp,338.95bp)  .. (6.7078bp,311.25bp) .. controls (-4.0586bp,296.0bp) and (0.31583bp,286.79bp)  .. (6.7078bp,269.25bp) .. controls (9.3361bp,262.04bp) and (14.208bp,255.29bp)  .. (N1);
  \draw (49.208bp,290.25bp) node {$\left(\begin{smallmatrix}0&\infty&\infty&\infty&\infty\cr
-1&-1&\infty&\infty&\infty\cr
\infty&\infty&0&\infty&\infty\cr
\infty&\infty&\infty&\infty&0\end{smallmatrix}\right)$};
  \draw (87.024bp,354.61bp) node {$$};
  \draw (20.413bp,248.44bp) node {$$};
  \draw [->] (N0) ..controls (137.78bp,364.37bp) and (152.71bp,361.62bp)  .. (152.71bp,350.25bp) .. controls (152.71bp,341.72bp) and (144.31bp,338.04bp)  .. (N0);
  \draw (196.71bp,350.25bp) node {$\left(\begin{smallmatrix}0&\infty&\infty&\infty&\infty\cr
-1&0&\infty&\infty&\infty\cr
\infty&\infty&0&\infty&\infty\cr
\infty&\infty&-1&-1&\infty\cr
\infty&\infty&\infty&\infty&0\end{smallmatrix}\right)$};
  \draw (130.89bp,364.51bp) node {$$};
  \draw (130.89bp,335.99bp) node {$$};
  \draw [->] (N1) ..controls (66.694bp,222.69bp) and (87.343bp,213.25bp)  .. (99.708bp,198.25bp) .. controls (111.8bp,183.58bp) and (117.26bp,162.27bp)  .. (N3);
  \draw (149.21bp,180.25bp) node {$\left(\begin{smallmatrix}0&\infty&\infty&\infty\cr
\infty&\infty&0&\infty\cr
\infty&\infty&\infty&0\end{smallmatrix}\right)$};
  \draw (58.203bp,233.83bp) node {$$};
  \draw (115.08bp,142.55bp) node {$$};
  \draw [->] (N1) ..controls (63.738bp,245.93bp) and (81.362bp,255.45bp)  .. (91.708bp,269.25bp) .. controls (105.25bp,287.3bp) and (110.46bp,313.22bp)  .. (N0);
  \draw (146.21bp,290.25bp) node {$\left(\begin{smallmatrix}0&\infty&\infty&\infty\cr
-1&0&\infty&\infty\cr
\infty&\infty&0&\infty\cr
\infty&\infty&-1&\infty\cr
\infty&\infty&\infty&0\end{smallmatrix}\right)$};
  \draw (57.021bp,246.44bp) node {$$};
  \draw (107.37bp,334.65bp) node {$$};
  \draw [->] (N2) ..controls (29.856bp,36.297bp) and (26.536bp,46.253bp)  .. (24.708bp,55.248bp) .. controls (12.048bp,117.54bp) and (8.378bp,136.09bp)  .. (21.708bp,198.25bp) .. controls (22.914bp,203.87bp) and (24.972bp,209.75bp)  .. (N1);
  \draw (51.708bp,126.75bp) node {$\left(\begin{smallmatrix}0&\infty&\infty&\infty\cr
-1&\infty&\infty&\infty\cr
\infty&0&\infty&\infty\cr
\infty&\infty&\infty&0\end{smallmatrix}\right)$};
  \draw (26.373bp,35.401bp) node {$$};
  \draw (25.271bp,218.22bp) node {$$};
%
\end{tikzpicture}


==> streams.tex <==

The recursor on Scott numerals can be adapted to other algebraic data
types like lists or trees. Surprisingly, it can also be adapted to some
coinductive data types. For instance, it is possible to encode streams
using the following definitions.

\begin{align*}
 \mathbb{S}(A) &= νK.∃S.\{\mathrm{hd} : S → A; \mathrm{tl} : S → K; \mathrm{st} : S\} \\
\mathrm{hd} &= λs.s.hd \; s.st\\
\mathrm{tl} &= λs.s.tl \; s.st\\
\mathrm{cons} &= λa\, l.\{\mathrm{hd}  = λu.a; \mathrm{tl}  = λu.l; \mathrm{st}  = ()\}
\end{align*}
In this definition of streams, the existentially quantified type is used
as an internal state of the stream. It needs to be provided in order to
compute an element of the stream. The order of the fixpoint and the
existential is essential to allow the typing of ``$\mathrm{cons}$''. The use of an
internal state is essential to keep strong normalization and add some
laziness to the data-type. In particular, a function call is required
to access a new element of the stream. The following definitions are
required to program a strongly normalizing co-iterator.

\begin{align*}
\mathrm{T}(A,P) &= ∀Y.(P × Y) → \{\mathrm{hd} : (P × Y) → A; \mathrm{tl} : Y; \mathrm{st} : P × Y\}\\
\mathbb{S}'(A,P) &= \{\mathrm{hd} : (P × \mathrm{T}(A, P)) → A; \mathrm{tl} : \mathrm{T}(A, P); \mathrm{st} : P × \mathrm{T}(A, P)\}\\
 \zeta   &\,: ∀A.∀P.(P → A) → ∀X.(P × X) → A \\
&= λf\, s.f \; s.1\\
 \delta  &\,: ∀A.∀P.(P → A) → (P → P) → \mathrm{T}(A, P) \\
&= λf\, n\, s.\{\mathrm{hd}  =  \zeta   \; f; \mathrm{tl}  = s.2; \mathrm{st}  = (n \; s.1, s.2)\}\\
\mathrm{coiter} &\,: ∀A.∀P.P → (P → A) → (P → P) →  \mathbb{S}(A)\\
&= λs\, f\, n.\begin{array}[t]{l}\LET A,P \ST f:P → A \IN\\ \left\{\setlength{\arraycolsep}{0.2em}\begin{array}{ll}\mathrm{hd}  &=  \zeta   \; f;\\
\mathrm{tl}  &=  \delta  \; f \; n;\\
\mathrm{st}  &= (s,  \delta  \; f \; n)\end{array}\right\} : \mathbb{S}'(A, P)\end{array}
\end{align*}

In these definitions, we use the same names as in the previous one to show the similarities.
The minimum type annotation for this program is to use the following subtyping relation:
$\mathbb{S}'(\mathrm{A}, \mathrm{P}) \subset  \mathbb{S}(\mathrm{A})$.
Here we gave also the type of $ \zeta  $ and $ \delta $, but it is not necessary.
As for Scott's numeral, a question arise about the meaning of the type
$∃P.\mathbb{S}'(\mathrm{A}, P)$.

One of the main difference in that we use here the native records of our language. For Scott's numeral, it is possible to use native sums, but we have to keep some function types to be able to program
a strongly normalisable recursor.
For the type $μN.[\mathrm{Z} | \mathrm{S} \of N]$, we were not able program such a recursor and we conjecture that it is impossible. However, if we encode the sum type using a record type, we can provide a recursor.
The type would then be
$N_t = μX.∀Y.\{\mathrm{z} : Y; \mathrm{s} : X → Y\} → Y$ which is very similar to the type of Scott's numeral.

%%% Local Variables:
%%% ispell-personal-dictionary: "~/.hunspell-en"
%%% ispell-local-dictionary: "british"
%%% End:


==> sum.tex <==

\begin{prooftree}
  \AxiomC{}
  \RightLabel{$$=$$}
  \UnaryInfC{$ \vdash x_2 ∈ \mathrm{A}(X_0) ⊆ \mathrm{A}(X_0)$}
  \RightLabel{$∀_r$}
  \UnaryInfC{$ \vdash x_2 ∈ \mathrm{A}(X_0) ⊆ ∀X.\mathrm{A}(X)$}
  \AxiomC{}
  \RightLabel{$$=$$}
  \UnaryInfC{$ \vdash x_1 \; x_2 ∈ K_0 ⊆ K_0$}
  \RightLabel{$→$}
  \BinaryInfC{$ \vdash x_1 ∈ ∀X.\mathrm{A}(X) → K_0 ⊆ \mathrm{A}(X_0) → K_0$}
  \AxiomC{}
  \RightLabel{$$=$$}
  \UnaryInfC{$ \vdash x_0 \; x_1 ∈ (\mathrm{B} → K_0) → K_0 ⊆ (\mathrm{B} → K_0) → K_0$}
  \RightLabel{$→$}
  \BinaryInfC{$ \vdash x_0 ∈ (\mathrm{A}(X_0) → K_0) → (\mathrm{B} → K_0) → K_0 ⊆ (∀X.\mathrm{A}(X) → K_0) → (\mathrm{B} → K_0) → K_0$}
  \RightLabel{$∀_l$}
  \UnaryInfC{$ \vdash x_0 ∈ \mathrm{Sum}(\mathrm{A}(X_0), \mathrm{B}) ⊆ (∀X.\mathrm{A}(X) → K_0) → (\mathrm{B} → K_0) → K_0$}
  \RightLabel{$∀_l$}
  \UnaryInfC{$ \vdash x_0 ∈ ∀X.\mathrm{Sum}(\mathrm{A}(X), \mathrm{B}) ⊆ (∀X.\mathrm{A}(X) → K_0) → (\mathrm{B} → K_0) → K_0$}
  \RightLabel{$∀_r$}
  \UnaryInfC{$ \vdash x_0 ∈ ∀X.\mathrm{Sum}(\mathrm{A}(X), \mathrm{B}) ⊆ \mathrm{Sum}(∀X.\mathrm{A}(X), \mathrm{B})$}
\end{prooftree}
\begin{center}
\begin{dot2tex}[dot,options=-tmath]
  digraph G {
  }
\end{dot2tex}
\end{center}


\begin{align*}
x_2 &= ε_{x ∈ \mathrm{A}(X_0)}(x_1 \; x ∉ K_0)\\
x_1 &= ε_{x ∈ ∀X.\mathrm{A}(X) → K_0}(x_0 \; x ∉ (\mathrm{B} → K_0) → K_0)\\
x_0 &= ε_{x ∈ ∀X.\mathrm{Sum}(\mathrm{A}(X), \mathrm{B})}(x ∉ \mathrm{Sum}(∀X.\mathrm{A}(X), \mathrm{B}))\\
X_0 &= ε_X(x_2 ∉ \mathrm{A}(X))\\
K_0 &= ε_K(x_0 ∉ (∀X.\mathrm{A}(X) → K) → (\mathrm{B} → K) → K)\\
%
\end{align*}

